Re-evaluating the Need for Multimodal Signals in Unsupervised Grammar Induction

Are multimodal inputs necessary for grammar induction? Recent work has shown that multimodal training inputs can improve grammar induction. However, these improvements are based on comparisons to weak text-only baselines that were trained on relatively little textual data. To determine whether multimodal inputs are needed in regimes with large amounts of textual training data, we design a stronger text-only baseline, which we refer to as LC-PCFG. LC-PCFG is a C-PFCG that incorporates em-beddings from text-only large language models (LLMs). We use a fixed grammar family to directly compare LC-PCFG to various multi-modal grammar induction methods. We compare performance on four benchmark datasets. LC-PCFG provides an up to 17% relative improvement in Corpus-F1 compared to state-of-the-art multimodal grammar induction methods. LC-PCFG is also more computationally efficient, providing an up to 85% reduction in parameter count and 8.8x reduction in training time compared to multimodal approaches. These results suggest that multimodal inputs may not be necessary for grammar induction, and emphasize the importance of strong vision-free baselines for evaluating the benefit of multimodal approaches.

==> sections/addition.tex <==
\clearpage
\section*{Limitations}
 While our experiments show that incorporating multimodal information does not improve performance on grammar induction, we can only draw conclusions about the tested methods of incorporating multimodal information. We note that we do not comprehensively test on all possible methods of incorporating multimodal cues, or all possible representations of multimodal information. It possible that there exists an untested method of incorporating multimodal information that \textit{would} benefit grammar induction. However, here we show that improvements in LLMs render prior methods of incorporating multimodal cues unnecessary for grammar induction.

 Moreover, here we evaluate grammar induction for English only. The benefits and limitations of incorporating multimodal information for grammar induction has not been studied for other languages. In future work, we hope our experiments can be extended to other languages, and investigate whether factors such as branching direction or word order flexibility affect the usefulness of multimodal information for grammar induction.


